Improved Safe Real-time Heuristic Search

A fundamental concern in real-time planning is the presence of dead-ends in the state space, from which no goal is reachable. Recently, the SafeRTS algorithm was proposed for searching in such spaces. SafeRTS exploits a user-provided predicate to identify safe states, from which a goal is likely reachable, and attempts to maintain a backup plan for reaching a safe state at all times. In this paper, we study the SafeRTS approach, identify certain properties of its behavior, and design an improved framework for safe real-time search. We prove that the new approach performs at least as well as SafeRTS and present experimental results showing that its promise is fulfilled in practice.

==> dead.tex <==
%Preliminaries
In this work we explore tradeoffs and efficiencies of proving safety in real time heuristic search. While much work has been done on experimental and theoretical analysis of real time search methods, to our knowledge there has been no additional exploration of proving safety in real time heuristic search beyond SafeRTS. Therefore, in addition to SafeRTS, we use as an alternative baseline comparison the popular real-time algorithm Local Search Space Learning Real-Time A* (LSS-LRTA*) \cite{koenig:crt}. This algorithm, described below, works well in directed state spaces and possesses desirable properties such as completeness in finite domains.


\todo[inline]{Remove theorem and define safety and dead-ends before.}
\begin{theorem}
Dead-ends or unsafe nodes are the dual of strong safe nodes.
\end{theorem}
\begin{proof}
The proof is trivial from the definition of these terms. A state is strongly safe if there exists a path to the goal from it and a state is a dead-end if no such path exists.
\end{proof}

